A BayeSN Distance Ladder: $H_0$ from a consistent modelling of Type Ia supernovae from the optical to the near infrared

The local distance ladder estimate of the Hubble constant ($H_0$) is important in cosmology, given the recent tension with the early universe inference. We estimate $H_0$ from the Type Ia supernova (SN~Ia) distance ladder, inferring SN~Ia distances with the hierarchical Bayesian SED model, BayeSN. This method has a notable advantage of being able to continuously model the optical and near-infrared (NIR) SN~Ia light curves simultaneously. We use two independent distance indicators, Cepheids or the tip of the red giant branch (TRGB), to calibrate a Hubble-flow sample of 67 SNe~Ia with optical and NIR data. We estimate $H_0 = 74.82 \pm 0.97$ (stat) $\pm\, 0.84$ (sys) km\,s$^{-1}$\,Mpc$^{-1}$ when using the calibration with Cepheid distances to 37 host galaxies of 41 SNe~Ia, and $70.92 \pm 1.14$ (stat) $\pm\,1.49$ (sys) km\,s$^{-1}$\,Mpc$^{-1}$ when using the calibration with TRGB distances to 15 host galaxies of 18 SNe~Ia. For both methods, we find a low intrinsic scatter $\sigma_{\rm int} \lesssim 0.1$ mag. We test various selection criteria and do not find significant shifts in the estimate of $H_0$. Simultaneous modelling of the optical and NIR yields up to $\sim$15\% reduction in $H_0$ uncertainty compared to the equivalent optical-only cases. With improvements expected in other rungs of the distance ladder, leveraging joint optical-NIR SN~Ia data can be critical to reducing the $H_0$ error budget.

==> scratch_suhail.tex <==
SN1998aq & 31.6001 & 0.0499 & 31.737 & 0.069 & -0.2042 & 0.0679 & 9.71 & N \\
SN2001el & 31.3267 & 0.0335 & 31.311 & 0.045 & -0.2823 & 0.583 & 10.69 & Y \\
SN2011fe & 29.0593 & 0.0447 & 29.135 & 0.045 & -0.1904 & 0.1885 & 10.18 & Y \\
SN2003du & 32.849 & 0.0333 & 32.919 & 0.063 & -0.7629 & 0.0521 & 8.6 & Y \\
SN1994ae & 32.0161 & 0.0542 & 32.072 & 0.049 & -0.4278 & 0.3097 & 9.69 & N \\
SN2007sr & 31.6288 & 0.0423 & 31.29 & 0.112 & -0.4095 & 0.325 & 10.05 & N \\
SN2015F & 31.4989 & 0.0257 & 31.511 & 0.053 & 0.651 & 0.327 & 7.212 & Y \\
SN2012fr & 31.3139 & 0.0257 & 31.307 & 0.057 & -1.0454 & 0.0178 & 6.737 & Y \\
SN2012ht & 32.0647 & 0.0333 & 31.908 & 0.043 & 0.9816 & 0.0514 & 8.06 & Y \\
SN2009ig & 32.8986 & 0.0351 & 32.497 & 0.081 & -1.1203 & 0.0072 & 10.56 & N \\
SN2013dy & 31.3127 & 0.0332 & 31.499 & 0.078 & -0.7884 & 0.5671 & 10.578 & Y \\
SN1995al & 32.2351 & 0.0542 & 32.498 & 0.09 & -0.9559 & 0.3603 & 9.87 & N \\
SN2012cg & 31.144 & 0.0427 & 31.08 & 0.292 & -0.7969 & 0.1832 & 8.467 & Y \\
SN2002fk & 32.4394 & 0.0345 & 32.523 & 0.055 & -0.3984 & 0.1006 & 9.94 & Y \\
SN2007af & 31.9505 & 0.0277 & 31.786 & 0.046 & 0.2225 & 0.3269 & 9.49 & Y \\
SN1990N & 31.7992 & 0.0523 & 31.532 & 0.071 & -0.7006 & 0.1696 & 10.14 & N \\
SN2011by & 31.7942 & 0.037 & 31.587 & 0.07 & -0.1088 & 0.2979 & 9.28 & Y \\
SN2005cf & 32.5644 & 0.039 & 32.263 & 0.102 & -0.4779 & 0.1231 & 9.47 & Y \\
SN1981B & 30.915 & 0.113 & 30.906 & 0.053 & 0.1009 & 0.222 & 10.47 & N \\

==> tables/H0_fitCase_fitOpt.tex <==
 \begin{table*}
    \centering
        \caption{Inferred value of $H_0$ and the absolute luminosity offset for the fiducial case and alternate case scenarios for the Cepheid calibrated distance ladder. We also report the intrinsic scatter term and the number of SNe in each of the calibrator and Hubble flow samples in every case.}

\begin{tabular}{|l|c|c|c|r|r|}
\hline
    Case & $H_0$    &   $\Delta M$ & $\sigma_{\rm int}$ & $N_{\rm calib}$ & $N_{\rm HF} $ \\
    & km\,${\rm s}^{-1}$\,${\rm Mpc} ^{-1}$ & mag & mag &  \\
    \hline
\textbf{ Fiducial} & \textbf{ XX $\pm$ 1.32} & \textbf{ YY $\pm$0.033} & \textbf{0.106 $\pm$ 0.016} & \textbf{18} & \textbf{55} \\
$z \geq 0.023$ & XX $\pm$ 1.456 & YY $\pm$ 0.033 & 0.116 $\pm$ 0.02 & 18 & 26 \\
NIR at max & XX $\pm$ 1.559 & YY $\pm$ 0.038 & 0.101 $\pm$ 0.019 & 9 & 32 \\
Restrictive Cut & XX $\pm$ 1.465 & YY $\pm$ 0.034 & 0.119 $\pm$ 0.018 & 18 & 40 \\


 \hline
    \end{tabular}
    \label{tab:h0_fitOpt}
\end{table*}

==> tables/calib.tex <==
\begin{table}
\caption{Calibrator sample used in this study with the Cepheid distances and the fitted distances using BayeSN.}
\begin{tabular}{|c|c|c|}
\hline 
SN & $\mu_{\rm Ceph}$ (mag) & $\mu_{\rm SN}$ (mag) \\
\hline 
SN1981B & 30.906 $\pm$ 0.104 & 30.906 $\pm$ 0.053 \\
SN1990N & 31.822 $\pm$ 0.11 & 31.532 $\pm$ 0.071 \\
SN1994ae & 32.047 $\pm$ 0.104 & 32.072 $\pm$ 0.049 \\
SN1995al & 32.281 $\pm$ 0.108 & 32.498 $\pm$ 0.09 \\
SN1998aq & 31.552 $\pm$ 0.106 & 31.737 $\pm$ 0.069 \\
SN2001el & 31.332 $\pm$ 0.094 & 31.311 $\pm$ 0.045 \\
SN2002fk & 32.403 $\pm$ 0.091 & 32.523 $\pm$ 0.055 \\
SN2003du & 32.86 $\pm$ 0.094 & 32.919 $\pm$ 0.063 \\
SN2005cf & 32.548 $\pm$ 0.096 & 32.263 $\pm$ 0.102 \\
SN2007af & 31.819 $\pm$ 0.094 & 31.786 $\pm$ 0.046 \\
SN2007sr & 31.402 $\pm$ 0.096 & 31.29 $\pm$ 0.112 \\
SN2009ig & 32.967 $\pm$ 0.093 & 32.497 $\pm$ 0.081 \\
SN2011by & 31.772 $\pm$ 0.095 & 31.587 $\pm$ 0.07 \\
SN2011fe & 29.016 $\pm$ 0.1 & 29.135 $\pm$ 0.045 \\
SN2012cg & 31.107 $\pm$ 0.092 & 31.08 $\pm$ 0.292 \\
SN2012fr & 31.032 $\pm$ 0.092 & 31.307 $\pm$ 0.057 \\
SN2012ht & 32.078 $\pm$ 0.095 & 31.908 $\pm$ 0.043 \\
SN2013dy & 31.396 $\pm$ 0.094 & 31.499 $\pm$ 0.078 \\
SN2015F & 31.506 $\pm$ 0.095 & 31.511 $\pm$ 0.053 \\
\hline
\end{tabular}
\label{tab:calib}
\end{table}

==> tables/prior_MCMC.tex <==
\begin{table}
    \centering
        \caption{Prior distribution for the parameters in the cosmological inference. We use the same wide prior for the intrinsic scatter term when treating the calibrator and Hubble flow samples separately.}

    \begin{tabular}{|c|c|}
    \hline 
    Parameter     &  Prior \\
        \hline 
    $H_0$     &    $\mathcal{U}$[50, 100]\\ 
    $M$    &   $\mathcal{U}$[-2, 2]\\
    $\sigma_{\rm int(, cal, HF)}$ & $\mathcal{U}$[0, 1] \\
    \hline 
    \end{tabular}
    \label{tab:prior_cosmo}
\end{table}
